HiDiGen: Hierarchical Diffusion for B-Rep Generation with Explicit Topological Constraints

Boundary representation (B-rep) is the standard 3D modeling format in CAD systems, encoding both geometric primitives and topological connectivity. Despite its prevalence, deep generative modeling of valid B-rep structures remains challenging due to the intricate interplay between discrete topology and continuous geometry. In this paper, we propose HiDiGen, a hierarchical generation framework that decouples geometry modeling into two stages, each guided by explicitly modeled topological constraints. Specifically, our approach first establishes face-edge incidence relations to define a coherent topological scaffold, upon which face proxies and initial edge curves are generated. Subsequently, multiple Transformer-based diffusion modules are employed to refine the geometry by generating precise face surfaces and vertex positions, with edge-vertex adjacencies dynamically established and enforced to preserve structural consistency. This progressive geometry hierarchy enables the generation of more novel and diverse shapes, while two-stage topological modeling ensures high validity. Experimental results show that HiDiGen achieves strong performance, generating novel, diverse, and topologically sound CAD models.

==> sec/problem_setup.tex <==
\section{Problem setup}



==> sec/two_stage_topo_construction.tex <==
% \section{Topology guided geometry construction}
% \label{sec: topo_construction}
% \subsection{Edge-face adjacency generation}
% The whole generation starts with a correct Edge-Face adjacency. We introduce a Transformer-based VAE for the generation of $\mathbf{EF}_i$.


% \subsubsection*{Transformer-based VAE}


% A set of learnable embeddings was introduced to the Transformer-based VAE for encoding the number of shared edges into continuous embeddings. Adn we employ the standard loss function used in VAE training, 

% \begin{equation}
% \begin{split}
% \mathcal{L} = 
% {} & \mathbb{E}_{\mathbf{z}_i \sim q_\phi(\mathbf{z}_i \mid \text{EF}_i^{\text{seq}})} \left[
% \mathrm{CE}\left( \text{EF}_i^{\text{seq}},\, \mathcal{D}_\theta(\mathbf{z}_i) \right)
% \right] \\
% {}+ & \mathrm{KL}\left( q_\phi(\mathbf{z}_i \mid \text{EF}_i^{\text{seq}}) \parallel \mathcal{N}(\mathbf{0}, \mathbf{I}) \right)
% \end{split}
% \end{equation}
% where $\mathcal{L}$ is the VAE training objective. The first term measures the reconstruction loss using cross-entropy (CE) between the input $\text{EF}_i^{\text{seq}}$ and the output of the decoder $\mathcal{D}_\theta$, given the latent variable $\mathbf{z}_i$ sampled from the encoder $q_\phi$. The second term is the Kullback–Leibler (KL) divergence that regularizes the encoder's distribution to be close to a standard normal prior $\mathcal{N}(\mathbf{0}, \mathbf{I})$.
\section{Topology and geometry generation}
% \begin{table*}[htbp]
% \centering

% \label{tab:quantitative_results}
% \begin{tabular}{llS[table-format=1.3]S[table-format=2.2]S[table-format=1.3]S[table-format=2.2]S[table-format=2.2]S[table-format=2.2]S[table-format=2.2]S[table-format=1.2]}
% \toprule
% \multicolumn{2}{l}{\textbf{Dataset}} 
% & {MMD $\downarrow$} & {COV $\uparrow$} & {JSD $\downarrow$} & {Valid $\uparrow$} & {Unique $\uparrow$} & {Novel $\uparrow$} & {CC $\uparrow$} & {MC $\uparrow$} \\
% \midrule

% \multirow{4}{*}{DeepCAD} 
% & DeepCAD          & 1.021 & 72.43 & 1.623 & 60.51 & 91.27 & 93.74 & 10.51 & 1.81 \\
% & BrepGen           & 0.874 & 71.12 & 1.584 & 69.27 & 99.08 & 99.54 & 9.30  & 0.86 \\
% & DGTBrepGen        & 0.867 & \best{76.86} & 1.504 & 73.29 & 99.13 & 99.21 & 9.78  & 0.73 \\
% & \textbf{HiDiGen} & \textbf{0.856} & 71.38 & \textbf{1.424} & \textbf{75.78} & \textbf{99.52} & \textbf{99.71} & \textbf{11.03} & \textbf{1.99} \\
% \midrule

% \multirow{3}{*}{ABC} 
% & BrepGen           & 1.543 & 66.37 & 2.377 & 53.48 & 97.64 & 98.57 & 10.76 & 1.37 \\
% & DGTBrepGen        & 1.455 & \best{68.21} & 2.024 & 63.53 & 98.86 & 99.02 & 11.45 & 1.06 \\
% & \textbf{HiDiGen} & \textbf{1.414} & 65.41 & \textbf{1.845} & \textbf{65.79} & \textbf{99.18} & \textbf{99.67} & \textbf{11.27} & \textbf{1.48} \\
% \bottomrule
% \end{tabular}
% \caption{Quantitative comparison of shape generation methods on DeepCAD and ABC datasets. Lower is better for MMD-CD and JSD; higher is better for COV, Valid, Unique, Novel, CC, and MC. Best results are \best{bolded}.}
% \end{table*}
\subsection{Topology generation}
Our topology generation framework operates in two seperate stages: $\mathbf{EF}_i$ generation and ($\mathbf{EV}_i$) generation stage, both implemented using an autoregressive Transformer architecture.

In the $\mathbf{EF}_i$ stage, we first encode the edge feature sequence $\mathbf{EF}_i^{\mathrm{seq}}$ into a latent representation using a Transformer encoder $\mathcal{E}_{\mathrm{EF}}$. A masked Transformer decoder $\mathcal{D}_{EF}$ then autoregressively reconstructs $\mathbf{EF}_i^{\mathrm{seq}}$ from this latent space. To encourage structured and disentangled representations, we formulate this process as a variational autoencoder (VAE), optimizing the standard VAE objective that combines reconstruction loss and KL regularization between the learned posterior and a prior distribution in the latent space.

For the $\mathbf{EV}_i$ stage, the Transformer encoder $\mathcal{E}_{\mathrm{EV}}$ processes edge embeddings $\mathbf{h}_i^{\mathrm{ef}}$, augmented with two special tokens $\langle \mathrm{L} \rangle$ and $\langle \mathrm{E} \rangle$. Each edge embedding consists of two components: context-aware edge features $\mathbf{h}_i^{\mathrm{ev}}$ and endpoint features. The context-aware features are extracted via a Graph Convolutional Network (GCN) that operates on the previously generated  information, effectively propagating contextual cues across the evolving topology. Following prior work, we decompose each edge into two directional node embeddings to enhance robustness in modeling cyclic or multi-way connections; this design facilitates more stable loop formation and is detailed in the Appendix. These refined embeddings are fed into $\mathcal{E}_{\mathrm{EV}}$ to produce contextualized edge representations.

The decoder $\mathcal{D}_{\mathrm{EV}}$ generates an edge connectivity sequence by attending to these contextual embeddings. Specifically, each index in the sequence $\mathbf{EV}_i^{\mathrm{seq}}$ is mapped to its corresponding contextual embedding, forming an ordered sequence that preserves the structural progression of edge connections. Positional encodings are added to retain sequential information, and the resulting sequence is processed by the Transformer decoder. Finally, a pointer network mechanism is applied at each decoding step to produce a probability distribution over candidate connections, enabling the model to autoregressively predict the most likely next edge connection given the current state.

\subsection{Geometry generation}
As detailed in Sec.~\ref{sec: geometry_representation}, our approach hierarchically generates geometric elements conditioned on the predicted topology and geometry. Specifically, face bounding boxes $\mathbf{B}_i$ and edge geometries $\mathbf{E}_i$ are generated under the guidance of the inferred face-edge adjacency structure $\mathbf{EF}_i$. Subsequently, face and vertex geometries are synthesized based on the full topological representation, including $\mathbf{EF}_i$ and $\mathbf{EV}_i$, along with previously generated geometric cues. Each stage of this  generation process benefits from rich contextual supervision.

We illustrate the geometry generation  using edge geometry as an example. Following the standard diffusion paradigm, we progressively add noise to the edge geometry tokens $\mathbf{E}_i$ and train a Transformer-based denoiser to predict the injected noise. A key aspect of our method is the integration of available prior information into the attention mechanism. In particular, we condition the denoising process on structural and spatial cues represented as $\mathbf{h}_i^b = \left[ \mathbf{t}_i^{fe} \right]$, where $\mathbf{t}_i^{fe}$ encodes the relationship between edges and their associated faces. This conditioning is incorporated into the attention computation, enabling the model to effectively leverage known face bounding box locations and explicit face-edge topological relationships, thereby enhancing structural coherence in the generated outputs. Fig. 10 illustrates an example of
 the generation process for edge geometry.
\subsubsection*{Post-Processing}
Since many surfaces correspond to
 basic types like planes or quadratic surfaces, when constructing the face geometry, we first attempt to fit the face’s
 boundary (discrete points sampled from the generated edge
 geometries) and interior (discrete points sampled from the
 generated face geometries) using basic primitives [19]. If
 the fitting error falls below a predefined threshold, we adopt
 the fitted primitives; otherwise, we resort to using the gen
erated B-spline surface (i.e., generated face geometries).
 Finally, we use OpenCascade [17] functions to seamlessly
 sew the generated topology and geometries into a coherent
 B-rep solid
